Polymer: Development Workflows as Software

Software development builds digital tools to automate processes, yet its initial phases, up to deployment, remain largely manual. There are two reasons: Development tasks are often under-specified and transitions between tasks usually require a translator. These reasons are mutually reinforcing: it makes little sense to specify tasks when you cannot connect them and writing a translator requires a specification. LLMs change this cost equation: they can handle under-specified systems and they excel at translation. Thus, they can act as skeleton keys that unlock the automation of tasks and transitions that were previously too expensive to interlink. We introduce a recipe for writing development workflows as software (polymer) to further automate the initial phases of development. We show how adopting polymer at Volvo, a large automotive manufacturer, to automate testing saved 2--3 FTEs at the cost of two months to develop and deploy. We close with open challenges when polymerizing development workflows.

==> acmart-primary/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> acmart-primary/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> attic/__dump <==
Put otherwise, under practical realities, how one can integrate LLMs and holistically gain meaningful efficiencies for a complete software engineering process? 

A loop in the process could have an iteration that last days to weeks, getting quick user feedback. The iteration could also last weeks to months, providing much slower feedback. At times, one loop could have complete responsibility for shipping a whole product to the customer. In more complex SE processes, separate loops could build parts of a product that another loop integrates and ships. 

\vspace{1mm}
\textbf{LLMs in embedded SE, a particular challenge} -- To a picture that is already complicated, we add another complication -- engineering embedded software. Compared many to other SE settings, embedded SE needs to pay a greater amount of attention to hardware aspects. For instance, in automotive embedded SE -- the standpoint from which we mainly articulate -- hardware takes wide meaning. It includes anything from electronic hardware to physical hardware like batteries, gearboxes, and pneumatic circuits. Going well beyond pure software focus, an automotive SE process therefore needs to integrate with the engineering lifecycle of dependent hardware. Under these conditions, inducting LLMs into a complete engineering process with demonstrable global gains becomes more challenging. We highlight some important conditions that increases the level of challenge. First, embedded SE can involve long integration chains. In vehicles, where embedded systems from different domains like driver assistance and energy efficiency coexist, hardware and software is developed and/or integrated at component, subsystem, and system levels. The span of a complete embedded SE process can therefore be much longer than other SE settings. Second, embedded SE usually needs to address many kinds of criticality. For example, depending upon its function, automotive SW may be required to meet timing, safety, or mission criticality demands. Ensuring that these demands are met is a process that spans the complete engineering process. Third, many embedded SE processes use methods and tools, that are often borrowed from other engineering disciplines. A good example is the sizeable influence of control systems and reliability engineering methods on automotive SE. Approaches taken by these allied disciplines -- the control loop or HW/SW co-design, for example -- are additional elements that an embedded SE needs to incorporate. The combination of these peculiarities makes embedded SE, particularly the automotive case, a much more complex enterprise. With all these extra elements of complexity, how does one induct LLMs into embedded SE and gain both local and global benefits? \looseness=-1

The inability in achieving best case outcomes could either be because tasks, where LLMs are applied, are not central to the larger process, or because the chosen LLM solution did not prioritize the necessary gain.

Taking local initiative, a team that executes some manual tasks may decide to use LLMs to automate them. Using either qualitative or quantitative means, they may also be able to demonstrate that this local initiative is beneficial to their team. If we, however, zoom out to consider the larger SE loop where this team plays a part, their local initiative could lead to different kinds of global effects. We sketch three potential scenarios. Best case, this local initiative, either singularly or in concert with other ones, is globally beneficial for the overall SE loop. Worse, this local initiative brings little or no global benefits. This could either be because the task itself is not central to the larger process, or because the chosen LLM solution did not prioritize the necessary gain. Let us consider the case that the team has set up a chatbot for accessing system documentation. After initial excitement, and after fresh inductees familiarize themselves with necessary documentation, the chatbot could fall into disuse. In this case, the marginal and ephemeral benefits of the chatbot may not justify the cost. Much worse, the local LLM initiative could end up harming a larger process. An example could be the team setting up a natural language chat interface for querying a database, because its members prefer this approach to using formal query languages. This local initiative favors a prompt-based interactive workflow instead of a code-based automatic workflow. The team may find using natural language queries more efficient but, arguably, the reduced level of automation harms the overall engineering process. \looseness=-1

As illustrated in Figure \ref{fig:swe-loops}, practical SE processes are a heterogeneous mix of tasks that are tedious, creative, and anything in between. Some of these tasks are executed manually, and others automatically. In some cases, a handful of teams execute a few SE loops to build and ship a product. In other cases, typically in large organizations, responsibility is diffuse with multiple teams executing multiple interdependent SE loops. A SE loop may be amenable to change, or it may be decades old, bearing the burden of considerable legacy. SE loops also evolve constantly, introducing, changing, and removing tasks, or reconfiguring their interdependencies. \looseness=-1

\vspace{1mm}
To a picture that is already complex, we add one more element -- the eccentricities of engineering embedded software. Compared many to other SE settings, embedded SE needs to pay a greater amount of attention to interdisciplinary aspects. For instance, in automotive SE -- the standpoint from which we mainly articulate -- interdisciplinary scope presents several additional challenges, some of which we highlight here. First, embedded SE can involve long integration chains. In vehicles, where embedded systems from different domains like driver assistance, propulsion, and energy efficiency coexist, hardware and software is developed and/or integrated at component, subsystem, and system levels. The span of a complete embedded SE process can therefore be much longer than other SE settings. Second, embedded SE usually needs to address many kinds of criticality. For example, depending upon its function, automotive SW may be required to meet timing, safety, or mission criticality demands. Ensuring that these demands are met is an undertaking that spans the complete engineering process. Third, a mix of disciplines means that embedded SE processes use methods and tools that are borrowed from other engineering disciplines. A good example is the sizeable influence of control systems and reliability engineering methods on automotive SE. Approaches taken by these allied disciplines -- like the control loop or HW/SW co-design -- are additional elements that an embedded SE needs to incorporate. The combination of these peculiarities makes embedded SE, particularly the automotive case, a much more complex enterprise.\looseness=-1

\vspace{1mm}
Under such complex and dynamic conditions, the instantaneous state of any SE processes -- embedded or not -- delicately balances a range of human, economic, and technical factors, usually in that order of priority. LLMs may offer powerful capabilities for SE, but how can they be gainfully incorporated into this delicate balance?\looseness=-1

\vspace{1mm}
\textbf{Current climate complicates LLM use in SE} --  The primary concern when using LLMs in SE is, of course, its reliability. If we, however, temporarily set this concern aside and take a broader look, we find that there are many additional concerns that complicate gainful incorporation of LLMs in SE. We now describe some of them. \looseness=-1

\begin{enumerate}[wide, labelindent=0pt]
    \item \textit{LLM assistance dominates imagination} -- ChatGPT and GitHub Copilot continue to dominate the imagination on generative AI in SE. While being powerful tools, chatbots and copilots epitomize LLM assistance -- a human is in the loop, prompting the LLM until a satisfactory response is reached. Assistance works best when executing a highly creative task like coding a new algorithm or brainstorming a new design. If, however, the task mainly requires judgement and not creativity, is an LLM assistant helpful? Take the example of an important but tedious task of reviewing whether APIs in an upcoming release comply with predefined naming conventions. Taking local initiative, a release team could use a chatbot or copilot to execute this task faster. But, from a global perspective, having a human in the loop for determining style compliance -- with or without assistance -- brings questionable overall gains. Scripting an LLM call (with necessary automatic evaluation) may be the best way forward. However, such is the dominance of the LLM assistance paradigm, particularly in organizations that are not on the leading edge of AI adoption, that automation is not always appreciated. With practical SE processes consisting of many tasks that do not reach creative heights, advocating LLM assistance alone does not lead to the best case outcome of globally gainful incorporation of LLMs in SE. \looseness=-1
    
    \vspace{1mm}
    \item \textit{Preference for natural language interfaces is heightened} -- The popularity of mainstream LLM assistants has led to an uptick in preference for Natural Language (NL) interfaces. In an SE processes, where many interfaces are meant to be used by programmers, how useful is an NL interface? Yet, inspired by LLM assistants that expose NL interfaces, there is significant popular demand for adopting the same in SE. Consider, for example, a team that needs to use a database, but with its members not being familiar with database query languages. This is not unusual in organizations where SE coexists with other disciplines. Taking local initiative, the team may decide to deploy an LLM layer that enables database interaction using NL queries. The team may find using NL queries more efficient, but favoring a prompt-based interactive workflow over a code-based automatic workflow reduces the level of automation. This can, in fact, harm global process efficiency. Granted, existing programming interfaces do not cater to every need, but favoring NL does not always lead to best case outcomes when incorporating LLMs into SE. \looseness=-1
    
    \vspace{1mm}
    \item \textit{Complex landscape challenges measurement} -- So far, we have discussed the problems faced when incorporating LLMs in very general terms. While we discuss the issue using notions like global versus local gains, complexity of SE processes, and current preferences in LLM use, we do so with the acute awareness that many of these notions are inherently difficult to define objectively. A SE task that appears discrete from one perspective could appear to be a complete process from another. Further, it is often difficult to define and measure gains when incorporating LLMs. Of late, there has been heightened attention \textcolor{red}{[cite]} on engineering productivity as being a major gain when using LLMs. But, as several studies \textcolor{red}{[cite]} point out, defining and measuring gains in SE productivity is no mean task. Finally, while one can recognize extra complexity in developing embedded SW, it is not clear how one can model this complexity and analyze its implications on LLM incorporation. With practitioners grappling with such fundamental questions, how does one approach the idea of gainfully using LLMs in (embedded) SE?
\end{enumerate}

LLM assistants dominates the imagination of LLMs in SE. LLM assistance requires a human engineer in the loop, prompting the LLM until a satisfactory response is reached. Such an assistance paradigm works best when the engineer is executing highly creative tasks like coding a new algorithm or brainstorming a new design. It is, however, of questionable value when executing a tedious task like reviewing whether new APIs comply with naming conventions. It may be more gainful to automate this task by scripting an LLM call. However, the dominance of the assistance paradigm -- particularly in organizations that are not on the leading edge of AI adoption -- increases the risk that a local initiative uses a chatbot/copilot to execute tedious tasks, resulting in high costs but meager global gains. Granted, LLM reliability is not yet up to the mark, but having engineers constantly verify its outputs, especially when executing tedious tasks, is not gainful from the standpoint of the overall SE process. Third, the popularity of mainstream LLM assistants has led to an uptick in preference for Natural Language (NL) interfaces. In an SE processes, where many interfaces are meant to be used by programmers, the utility of an NL interface is questionable. Yet, inspired by LLM assistants that expose NL interfaces, there is significant popular demand for adopting the same in SE. Consider, for example, a team that needs to use a database, but with its members not being familiar with database query languages. This is not unusual in organizations where SE coexists with other disciplines. Taking local initiative, the team may decide to deploy an LLM layer that enables database interaction using NL queries. The team may find using NL queries more efficient, but favoring a prompt-based interactive workflow over a code-based automatic workflow could reduce global process efficiency. Overall, while there are genuine shortcomings in LLM capabilities, current trends like the preference for assistance and NL interfaces make globally gainful LLM incorporation even more challenging. \looseness=-1

Another example is drawing inspiration form popular LLM assistants and deploying Natural Language (NL) interfaces for interacting with digital systems. Say a local initiative deploys an NL interface for accessing databases. The preference for a prompt-based interactive workflow over a code-based automatic workflow that this local initiative favors may actually worsen global process efficiency. 

==> attic/_dump <==
% The workflow itself can be considered as a directed acyclic graph with tasks as nodes. Then, let us define an edge in the graph $L_{ij}$ connecting tasks $T_i$ and $T_j$ as an \textit{interlinking} activity, examples of which include steps like coordination, gating, or hand-off. Unlike tasks, interlinks tend to be under-specified, but they nevertheless play a crucial glue role in keeping the process together. What does applying \dews, or \dews-ing, such a workflow practically mean?

% Clearly, applying \dews to streamline this workflow means automating as many tasks and interlinks as possible. What does this mean in practice? 

%Despite its advantages, realizing \dews by writing development workflows as code can be challenging. We highlight two important dimensions of this challenge. First, workflows must be decomposed into discrete tasks, inputs and outputs of each task must be formalized, and the task itself must be made executable. These steps are not always simple and could involve substantial cost and effort. Second, not all tasks in a workflow are concretely definable. Some tasks, particularly those that produce concrete deliveries like code or test cases, are well-defined and relatively easy to formalize. Other tasks like coordination or hand-off are under-specified, but they constitute the glue 

%In fact, we posit that tasks in a workflow fall into two broad types --- main tasks and connector tasks. We define main tasks as those that are well-specified and lead to concrete deliveries like code or test cases, making them relatively easy to formalize. In contrast, we define connector tasks as those that do not necessarily lead to tangible deliveries but act as glue to keep the process flowing. Coordination or hand-off are typical examples of connector tasks and their under-specified nature makes them particularly vexing to formalize. Due to these challenges, if a workflow can be made executable at all, it starts out being brittle and matures slowly, requiring continuous refinement, sometimes over long time periods, to make it robust. 

%Isolated attempts rarely go beyond the initial brittle phase or, worse, simply fail to materialize.

% This creates sufficient scale for the SE community to put in enormous effort and conventionally engineer the deep technology stack necessary for operations. 
%and, worse case, so unique that conventional automation becomes prohibitively expensive.

% On the other hand, several obstacles also immediately surface. Conceptually, unlike SW operations, SW development involves less-standard tasks, deals with a wider design space, and is highly domain dependent. Practically, further, it is challenging to implement certain development tasks as software. Tasks like choosing test inputs for the air suspension system, or searching for parameters to calibrate the engine controller are not trivial to code. It often takes enormous effort to develop and maintain algorithms or heuristics for automating arcane development tasks. Given that such obstacles can cancel out any of the potential benefits, why do we make a case for SW-defined development workflows? We argue that the time for such an idea is ripe because of a crucial tipping factor - the advent of Large Language Models (LLMs). We reason that an LLM's ability to be a general purpose tool that solves a wide range of SW development tasks allows us to left-shift into the head-end of SE, and write more development workflows as software.

%We deliberate upon the feasibility of this hypothesis, and the recipe derived from it, on an example software system drawn from industry to illustrate the opportunities and challenges of realizing LLM-enabled SW-defined development workflows.

%From each of these perspectives, conventional automation stands in stark contrast. In the conventional approach, automation is largely addressed on a task-basis, and is achieved by developing some rule-based implementation, which can be costly and time-consuming. Further, the conventional approach requires formalizing input and output data structures, which is both expensive and brittle. Not only is data parsing error-prone, the proliferation of data formats leads to tedious data wrangling steps in workflows.

% \vspace{1mm}
% We now introduce a running example, drawn from industry, to deliberate upon this question. \spapi (see Figure \ref{fig:spapi-overview}) is a simple web server deployed in trucks manufactured by a leading vehicle company. It provides RESTful APIs that allows clients (like tablet applications) access and manipulate vehicle state. For instance, \spapi exposes the \texttt{/speed} endpoint to read the vehicle speed and the \texttt{/climate} endpoint to adjust cabin climate. Like many other software units in the larger in-vehicle embedded system, \spapi operation is automatic. SW-defined operations continuously integrate new \spapi functionality, regularly run regression tests, and make new releases. However, if one shifts left into testing, one would observe that \spapi testing is a largely manual activity that requires a dedicated team of 2-3 full-time engineers. In the case of SPAP, as we show later, the complete contrast between automatic SW-defined operation and manual testing arises not from any inherent technical complexity, but from a need to manage complex system documentation.

% \input{figures/spapi-overview.tex}

%In recent years, we have seen the rise of a powerful technology -- generative AI and, particularly, Large Language Models (LLMs) -- which is revolutionizing SE. LLMs have been applied for assisting or automating discrete SE tasks like requirements engineering, software design, coding, and testing \cite{DBLP:conf/fose-ws/FanGHLSYZ23, DBLP:journals/corr/abs-2308-10620}. Witnessing the rapid increase of LLM applications in discrete SE tasks, this paper fundamentally considers the question -- can LLMs help organizations reduce global SE process inefficiencies by being the skeleton key that fixes a multitude of local task-level inefficiencies? \looseness=-1

%Considering the success of SW-defined operations, we ask - is the time to shift left from operations and also write \textit{development} workflows as software? %That is, is it time for defining specification, implementation, and verification workflows as software?

%Despite being a standard RESTful web server, why is the level of test automation so low? The root of the problem is that \spapi acts as the single interface to a highly distributed in-vehicle state system. The correspondence between properties $(p_i, q_i)$ of an API object $E$ and vehicle states $(r_i, s_i)$, which testers rely upon, is spread over at least five different sources of documentation. Making matters worse, the responsibility for maintaining specification is diffuse. Several inconsistencies inevitably creep in, and testers navigate them manually. To alleviate this tedium, let us consider automating this workflow by writing it as code. \looseness=-1
% This is because the specification of correspondence between API properties and vehicle states is spread over five sets of documentation. Two separate sets of documentation hold information about endpoints and VV states respectively. Further, in the vehicle embedded system, state is accessed by reading/writing Controller Area Network (CAN) signals. That is, a state like \texttt{ACState} is accessed by reading a CAN signal \texttt{APIACModeRqst} and a third set of documents hold a list of CAN signals. The correspondence between API properties and vehicle state are themselves specified in two other sets of documents that capture links between the three base set of documents. Adding to the complexity of having five separate sets of documentations, mappings between them are highly unstructured --- they are fuzzy, not always complete, and are expressed in different ways, including as pseudocode. Such lack of structure means that there is no uniform mechanism to query and map specifications, making it difficult to implement \texttt{map\_api\_obj\_to\_vehicle\_state}. Thus, a SW-defined workflow remains unrealized, and tedious manual work becomes the norm. \looseness=-1

% , a list of which is held in a third set. Linking these three sets are two other documents, one each for capturing API $\rightarrow$ CAN, and CAN $\rightarrow$ VV links.

% We have already seen that endpoint objects $E = \{(k_i, v_i)\}_{i=1}^{N_E}$ with properties $k_i$ and value $v_i$ are captured in OpenAPI specifications. The corresponding vehicle state $V = \{(k^{\prime \prime}_i, v^{\prime \prime}_i)\}_{i=1}^{N_V}$ is documented separately. Further, in the vehicle embedded system, state is accessed by reading/writing Controller Area Network (CAN) signals. So, the link between endpoints and vehicle states are CAN signals $C = \{(k^{\prime}_i, v^{\prime}_i)\}_{i=1}^{N_C}$, which are also documented separately.

% $(k_i, v_i)$, CAN signals $(k^{\prime}_i, v^{\prime}_i)$,  and vehicle states $(k^{\prime \prime}_i, v^{\prime \prime}_i)$ is spread over multiple sets of documentation. Making matters worse, mappings are highly unstructured --- they are fuzzy, not always complete, and are expressed in different ways, including as pseudocode. Such lack of structure means that there is no uniform mechanism to query and map specifications, making it difficult to implement \texttt{map\_api\_obj\_to\_vehicle\_state}. Thus, a SW-defined workflow remains unrealized, and tedious manual work becomes the norm. \looseness=-1
%API object $E = \{(k_i, v_i)\}_{i=1}^{N_E}$ and associated vehicle states $V = \{(k^{\prime \prime}_i, v^{\prime \prime}_i)\}_{i=1}^{N_V}$. In the vehicle embedded system, state is accessed by reading/writing Controller Area Network (CAN) signals. So, to write a test case, testers first use the OpenAPI endpoint specification to craft an API object $E$. They then refer to 3-5 additional specifications to first map the API properties to corresponding CAN signals $C = \{(k^{\prime}_i, v^{\prime}_i)\}_{i=1}^{N_C}$, and then finally to vehicle states $V$. In the acceptance testing setup, vehicle state is mocked by a Virtual Vehicle (VV) system, which holds all vehicle states in a table. So, testers write test cases to \texttt{GET}/\texttt{PUT} the API object $E$ and check the VV state table to see if the vehicle state corresponds to $V$. 

% At the most granular level, a SE process consists of discrete tasks like design, implementation, or verification. At higher levels, these tasks link up to form development workflows that build and deliver components or subsystems. 

% Shipping a complete product to the customer usually requires several development workflows to come together and integrate their respective deliveries.

% , some of them at a global scale catering to millions of users. Even in a HW-intensive process like vehicle embedded systems, SW automation is commonplace. SW-defined workflows continuously integrate new features, run regression tests, make releases, and download them into vehicles

% Such is its level of maturity that operations is considered as a distinct, principled SE discipline.

% It may take weeks to know whether a new feature works as intended in the target environment. By extension, it may take months to make product updates and years to introduce a new product. 

%So, if we were to construct a distribution of SE workflows arranged by their cross-domain prevalence, operations surely converge in its bulky `head'.

% In the acceptance testing setup, vehicle state is mocked by a Virtual Vehicle (VV) system, making it easy to read/write states. 

% When developing a cyberphysical system like a vehicle, for instance, SE complexity is quite high. and handling challenges across the spectrum of SE activities. Under such difficult conditions, it is therefore quite a challenge to run a high cadence SE process and deliver high quality products.

%\textbf{Specification is a vortex of coordination.} When \texttt{spapi} architects identify the need for an endpoint like \texttt{/climate} with a property \texttt{acMode}, they first define its interface as an OpenAPI specification. Then, using domain knowledge, they identify that this endpoint has a natural connection with the climate control system. Best case, climate states are well documented and states that correspond to properties are easily identified. But quite often, state documentation is incomplete, out of date, or even absent. Therefore, \spapi architects reach out to the climate team to jointly identify \texttt{ACState} as the vehicle state that best corresponds to the API property \texttt{acMode}. Adding to the complexity, vehicle states are accessed by reading and writing Controller Area Network (CAN) signals. So, \spapi architects additionally reach out to a signal definition team to identify \texttt{APIACModeStatus} and \texttt{APIACModeRqst} as signals to respectively read and write \texttt{ACState}. After spending several hours on average coordinating, \spapi architects specify the mapping between one property-signal-state set as informal text (Figure \ref{fig:spapi-endpoint-example}(a)). With \spapi exposing a few hundred APIs and few thousand attributes, \Volvo spends thousands of person hours on API specification alone.\looseness=-1


==> attic/automation-recipe.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{./figures/automation-recipe.jpg}
    \caption{Our recipe -- automate SE loops by decomposing and writing workflows as code that runs on a compound AI SE system}
    \label{fig:automation-recipe}
\end{figure}

==> attic/left-shift.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{./figures/left-shifting-programmed-automation.jpg}
    \caption{Using LLMs as a skeleton-key, we propose that more and more development workflows can be written as software}
    \label{fig:left-shift}
\end{figure}

==> attic/swe-loops.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{./figures/swe-loops.jpg}
    \caption{In real world settings, a set of dependent SE loops come together to build and ship a product to the customer. Some tasks in these loops are executed manually, and others automatically. The state of these loops are also constantly evolving. Under such complex and dynamic conditions, how can LLMs be incorporated to gain overall efficiencies?}
    %\label{fig:swe-loops}
\end{figure}

==> attic/teaser.tex <==
\begin{teaserfigure}
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{./figures/swe-loops.jpg}
        \label{fig:swe-loops}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=1.0\linewidth]{./figures/automation-recipe.jpg}
        \label{fig:automation-recipe}
    \end{subfigure}
    \caption{(a) In real world settings, multiple Software Engineering (SE) loops come together to build and ship a product. Tasks in these loops are executed either manually or automatically, and the state of loops evolve constantly. Under such complex and dynamic conditions, how can AI be used to gain efficiencies not just at task-level but at the overall process level? (b) We propose an organizing principle for demonstrably gainful use of generative AI in SE -- maximizing automation, with the target end state of complete automation. We then propose a recipe to realize this end state -- decomposing the workflow into discrete tasks, and writing this workflow as code that runs on a compound AI SE system that combines LLMs with conventional automation. \looseness=-1}
    \label{fig:overview}
\end{teaserfigure}

==> figures/spapi-overview.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{./figures/spapi-overview.jpg}
    \caption{\spapi is an in-vehicle web server. It exposes RESTful APIs that allow clients to access vehicle state.}
    \label{fig:spapi-overview}
\end{figure}

==> figures/sw-defined-dev-workflows.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{./figures/sw-defined-dev-workflows.jpg}
    \caption{We propose that software engineering complexity is better managed by writing development workflows as software. The advent of Large Language Models (LLMs), we argue, has drastically reduced the threshold to achieve this.}
    \label{fig:sw-defined-workflows}
\end{figure}
